3D Ensemble-Based Online Oceanic Flow Field Estimation for Underwater Glider Path Planning

Estimating ocean flow fields in 3D is a critical step in enabling the reliable operation of underwater gliders and other small, low-powered autonomous marine vehicles. Existing methods produce depth-averaged 2D layers arranged at discrete vertical intervals, but this type of estimation can lead to severe navigation errors. Based on the observation that real-world ocean currents exhibit relatively low velocity vertical components, we propose an accurate 3D estimator that extends our previous work in estimating 2D flow fields as a linear combination of basis flows. The proposed algorithm uses data from ensemble forecasting to build a set of 3D basis flows, and then iteratively updates basis coefficients using point measurements of underwater currents. We report results from experiments using actual ensemble forecasts and synthetic measurements to compare the performance of our method to the direct 3D extension of the previous work. These results show that our method produces estimates with dramatically lower error metrics, with and without measurement noise.

==> intro_notes_collected.tex <==
\begin{itemize}
    \item Underwater gliders can be so much more useful than they are now: ocean science, defence, energy.
    \item Why aren't they being used as much as they could in these fields (and others)? One major issue is accurate navigation and planning algorithms. Gliders present a special problem: they have much lower thrust, so the currents affect us much more.
    \item Name drop our planning papers?
    \item A major bottleneck is oceanic flow field estimation.
    % \item A valuable source of data for estimation are the \textit{ensemble forecasts}.
%     \item Ensemble forecasts, a standard tool used in meteorology, are composed of many members, each of which is a flow field prediction produced by a deterministic physical simulation from slightly different initial conditions.
% The initial conditions are informed by relatively recent sensor measurements and their respective sensor models.
% Together, the members of the ensemble forecast comprise a small sample of possible future weather conditions given the current sensor measurements.
    % \item In this paper we address oceanic flow field estimation using \textit{ensembles} and online measurements from robots.
%     \item \fk{Downplay compression. Relegate to a sentence or two in discussion.} Another relevant engineering concern for deployment of a flow field estimator is the amount of data required to specify the model. 
% It is important for vehicles at sea to receive the latest flow field estimates; however, this is constrained by the bandwidth of the communications available.
% Current satellite communications bandwidth is on the order of kilobits per second; sending a large or high-resolution flow field may take a long time.
% As such, a desirable property of a flow field estimate is a compact representation.

\item In this paper, we propose a 3D extension to a 2D flow field estimator which takes an ensemble forecast and measurement data. Motivated by a physics-based insight, we also make a variation to the algorithm to improve estimation accuracy.
    % \item Can we argue that going from 2D to 3D is an enlargement of span? And that bigger span is better, and our method provides an even bigger span than naive 3D?
\end{itemize}

\subsection{Our approach/novelty}
We build upon an existing work which estimates 2D flow field using an ensemble forecast and sensor measurements~\cite{to2021}.
We improve upon this work not only by extending the methods in that paper to the 3D case, but more importantly, alter the algorithm according to a physics-based insight, resulting in improved accuracy. 
%with a more compact representation.


% Motivated by this, we consider 3D flow fields as a family of depth-varying 2D flow fields.
% This allows estimating the flow field at each depth by using basis flow fields generated not only from the ensemble data of the corresponding depth, but from other depths as well.
% This ``cross-depth'' availability of flow fields increases the span of the basis, and hence reduces the error due to the true flow field being outside the span of the basis.
% Additionally, the use of the singular value decomposition allows truncation of low-power modes that do not contribute significantly, resulting in a compact estimate.

% In Section \ref{sec:related_work} we discuss related work in the literature, and present our problem formulation and approach in Sections \ref{sec:problem_formulation} and \ref{sec:approach}, respectively.
% Results from simulation experiments are discussed in \ref{sec:results_and_discussion}, with a short conclusion in \ref{sec:conclusion}.

